Johnsen-Rahbek Capstan Clutch: A High Torque Electrostatic Clutch

In many robotic systems, the holding state consumes power, limits operating time, and increases operating costs. Electrostatic clutches have the potential to improve robotic performance by generating holding torques with low power consumption. A key limitation of electrostatic clutches has been their low specific shear stresses which restrict generated holding torque, limiting many applications. Here we show how combining the Johnsen-Rahbek (JR) effect with the exponential tension scaling capstan effect can produce clutches with the highest specific shear stress in the literature. Our system generated 31.3 N/cm^2 sheer stress and a total holding torque of 7.1 Nm while consuming only 2.5 mW/cm^2 at 500 V. We demonstrate a theoretical model of an electrostatic adhesive capstan clutch and demonstrate how large angle (theta > 2pi) designs increase efficiency over planar or small angle (theta < pi) clutch designs. We also report the first unfilled polymeric material, polybenzimidazole (PBI), to exhibit the JR-effect.

==> scrap.tex <==
An important design factor for the capstain break is the yeild stress of the band materials. The cross sectional area of the band is $l h$ where $h$ is the thickness of the band. The tension in the band is $T_{load}$ so $\sigma_{max} = \frac{T_{load}}{(l h)}$ 
IF we assume $T_{hold} << 1$ $T_{load} = \beta l r (e^{\mu\theta}-1)$ where $\beta l r = \alpha$ so dividing by the area,

\begin{equation}
\sigma_{max} =  \frac{r}{h} \beta (e^{\mu\theta}-1)
\label{eqn:stress}
\end{equation}

It is important to note that the stress in the band is not a function of its width, but the output force is a function of width. Therefore If you are operating at the maximum limit of the band material, using a wider band can linearly improve performance. 

The torque we output is $\tau_{load} = T_{load} r =  l r^2 \beta (e^{\mu\theta}-1)$
Substituting in $\sigma_{max}$ we get $\tau_{max} = l h r \sigma_{max}$. Therefor for a fixed maximum stress of a band material, we can linearly improve the output torque by increasing the band thickness, width or the radius of the clutch. 

This makes it clear that in a capstan design, we can always reach the limit of the band material by increasing the wrap angle till $T_{load} = T_{max}$ At which point increasing break performance will depend on selecting a different band material, or linear improvements based on geometric trade offs.  Increasing the performance of dielectric material will improve the $\beta$ term and will more efficiently convert power or voltage into holding force and a smaller radius shaft will generate the same holding torques. 


